Revisiting Weak-to-Strong Consistency in Semi-Supervised Semantic Segmentation

In this work, we revisit the weak-to-strong consistency framework, popularized by FixMatch from semi-supervised classification, where the prediction of a weakly perturbed image serves as supervision for its strongly perturbed version. Intriguingly, we observe that such a simple pipeline already achieves competitive results against recent advanced works, when transferred to our segmentation scenario. Its success heavily relies on the manual design of strong data augmentations, however, which may be limited and inadequate to explore a broader perturbation space. Motivated by this, we propose an auxiliary feature perturbation stream as a supplement, leading to an expanded perturbation space. On the other, to sufficiently probe original image-level augmentations, we present a dual-stream perturbation technique, enabling two strong views to be simultaneously guided by a common weak view. Consequently, our overall Unified Dual-Stream Perturbations approach (UniMatch) surpasses all existing methods significantly across all evaluation protocols on the Pascal, Cityscapes, and COCO benchmarks. Its superiority is also demonstrated in remote sensing interpretation and medical image analysis. We hope our reproduced FixMatch and our results can inspire more future works. Code and logs are available at https://github.com/LiheYoung/UniMatch.

==> table/ablation_fp_only.tex <==
\begin{table}[H]
	\centering
	\small
	
	\begin{tabular}{l|ccccc|ccc}
		\toprule

		Perturbation Level & 92 & 183 & 366 & 732 & 1464 & 1/16 & 1/8 & 1/4 \\

		\midrule
		\midrule
		
		Image Level Alone (FixMatch) & 63.9 & 73.0 & 75.5 & 77.8 & 79.2 & 74.1 & 75.9 & 76.4 \\
		
		Feature Level Alone & 66.0 & 69.6 & 74.0 & 77.3 & 78.9 & 73.7 & 74.5 & 76.4 \\
		
		\midrule
		
		Unified Levels (UniPerb) & 72.0 & 75.8 & 77.5 & 79.3 & 80.1 & 76.0 & 76.9 & 76.6 \\
		
		\bottomrule
	\end{tabular}
	\caption{Results (\%) of only using \emph{single} perturbation level, either image-level perturbations (original FixMatch) or feature-level perturbations. These results are obtained from the Pascal dataset with DeepLabv3+ and ResNet-101. We also provide results of our UniPerb (Unified Levels) as a reference, which unifies the two different levels of perturbations.}
	\label{table:ablation_fp_only}
\end{table}


==> table/ablation_num_of_strong.tex <==
\begin{table}[H]
	\centering
	\small
	
	\begin{tabular}{l|ccccccc}
		\toprule

        \multirow{2}{*}{Number of labeled images} & \multicolumn{7}{c}{Number of image-level perturbation streams} \\
        
        \cmidrule{2-8}
        
		~ & 1 (FixMatch) & 2 (DusPerb) & 3 & 4 & 5 & 6 & 7 \\

		\midrule
		\midrule
		
		High-quality set: 732 & 77.8 & 78.1 & 78.8 & 78.9 & \textbf{79.1} & 78.7 & 78.4 \\
		
		Blended set: 662 (1/16) & 74.1 & 75.3 & 75.4 & 76.1 & 76.0 & \textbf{76.7} & 76.3 \\

		\bottomrule
	\end{tabular}
	\caption{The performance (\%) change with respect to the number of image-level strong perturbation streams.}
	\label{table:ablation_num_of_strong}
\end{table}


==> table/ablation_uniperb_dual.tex <==
\begin{table}[H]
	\centering
	\small
	
	\vspace{1mm}
	
	\begin{tabular}{l|ccccc|ccc}
		\toprule

		Method & 92 & 183 & 366 & 732 & 1464 & 1/16 & 1/8 & 1/4 \\

		\midrule
		\midrule
		
		Single-Stream FP (UniPerb) & 72.0 & 75.8 & 77.5 & 79.3 & 80.1 & 76.0 & 76.9 & 76.6 \\
		
		Dual-Stream FP & \textbf{73.4} & \textbf{77.1} & \textbf{78.5} & \textbf{79.6} & \textbf{80.4} & \textbf{76.2} & \textbf{77.0} & \textbf{76.8} \\
		
		\bottomrule
	\end{tabular}
	\caption{Effectiveness of dual-stream perturbations at the feature level (\%). FP here denotes feature perturbation. Same as the single-stream FP (UniPerb), the dual-stream FP also contains one stream for image-level strong perturbations.}
	\label{table:ablation_uniperb_dual}
\end{table}

